Accelerated Distributed Nesterov Gradient Descent

This paper considers the distributed optimization problem over a network, where the objective is to optimize a global function formed by a sum of local functions, using only local computation and communication. We develop an Accelerated Distributed Nesterov Gradient Descent (Acc-DNGD) method. When the objective function is convex and $L$-smooth, we show that it achieves a $O(\frac{1}{t^{1.4-\epsilon}})$ convergence rate for all $\epsilon\in(0,1.4)$. We also show the convergence rate can be improved to $O(\frac{1}{t^2})$ if the objective function is a composition of a linear map and a strongly-convex and smooth function. When the objective function is $\mu$-strongly convex and $L$-smooth, we show that it achieves a linear convergence rate of $O([ 1 - C (\frac{\mu}{L})^{5/7} ]^t)$, where $\frac{L}{\mu}$ is the condition number of the objective, and $C>0$ is some constant that does not depend on $\frac{L}{\mu}$.

==> sec_3_review_and_motivation.tex <==


\section{Algorithm development: Motivation}\label{sec:motivation}
In this section, we will briefly review distributed first-order optimization algorithms that are related to our algorithm and discuss their limitations which motivates our algorithm development. In particular, we will formally provide an impossibility result regarding the limitations. Lastly we will discuss the literature that motivates the idea of harnessing the smoothness from history information. 
  
\subsection{Review of Distributed First-Order Optimization Algorithms}

	


\subsection{Harnessing Smoothness via History Information}\label{subsec:history_info}

